What's Hidden in a One-layer Randomly Weighted Transformer?

We demonstrate that, hidden within one-layer randomly weighted neural networks, there exist subnetworks that can achieve impressive performance, without ever modifying the weight initializations, on machine translation tasks. To find subnetworks for one-layer randomly weighted neural networks, we apply different binary masks to the same weight matrix to generate different layers. Hidden within a one-layer randomly weighted Transformer, we find that subnetworks that can achieve 29.45/17.29 BLEU on IWSLT14/WMT14. Using a fixed pre-trained embedding layer, the previously found subnetworks are smaller than, but can match 98%/92% (34.14/25.24 BLEU) of the performance of, a trained Transformer small/base on IWSLT14/WMT14. Furthermore, we demonstrate the effectiveness of larger and deeper transformers in this setting, as well as the impact of different initialization methods. We released the source code at https://github.com/sIncerass/one_layer_lottery_ticket.

==> algo.tex <==
\begin{algorithm}[t]
\DontPrintSemicolon
\caption{Hessian AWare Quantization}
\label{alg:hq}
    \SetAlgoLined
    \KwInput{Block-wise Hessian eigenvalues $\lambda_i$ (computed from~\aref{alg:power_iteration}), and block size $n_i$ 
    for $i=1,\cdots,b$.

    }

    \For(\tcp*[h]{Compute Quantization Precision}){i $=1,2,\ldots, b$}{

        $S_i = \lambda_i/n_i$ \tcp*{See~\eref{eqn:define_S}}
    }
    
    
    Order $S_i$ in descending order and to determine relative quantization precision for each block.
    
    Compute $\Delta W_i$ based on~\eref{eqn:quantization_function}.

    \For(\quad \quad \quad\quad\quad \tcp*[h]{Fine-Tuning Order}){i $=1,2,\ldots, b$}{
       $\Omega_i = \lambda_i\|\Delta W_i\|^2$ \tcp*{See~\eref{eqn:define_O}}
    }
    
    Order $\Omega_i$ in descending order and perform block-wise fine-tuning
\end{algorithm}





==> packages.tex <==

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{times}
\usepackage{soul}
\usepackage[utf8]{inputenc}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{booktabs}
\usepackage{adjustbox}




% \usepackage[colorlinks=true,
% citecolor=blue,
% filecolor=black,
% linkcolor=blue,
% urlcolor=blue]{hyperref}

\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{booktabs} % for professional tables


% Optional math commands from https://github.com/goodfeli/dlbook_notation.
% \input{math_commands.tex}

\usepackage{multirow}
\usepackage{paralist}

\usepackage{booktabs} % for professional tables
\usepackage{multicol}
\usepackage{diagbox}

\usepackage[ruled,noend]{algorithm2e}
\newcommand{\theHalgorithm}{\arabic{algorithm}}
\newcommand\mycommfont[1]{\scriptsize\ttfamily\textcolor{blue}{#1}}
\SetCommentSty{mycommfont}

\usepackage{here}

\usepackage{amsmath,amssymb,amsfonts,amsbsy,amsfonts,latexsym}
\usepackage{multirow}
\usepackage{makecell}
% \usepackage[labelfont=bf,textfont=it,belowskip=0pt,aboveskip=5pt,tableposition=top]{caption}
\usepackage{xcolor}
\usepackage{colortbl}
\let\proof\relax
\let\endproof\relax


\definecolor{colorA}{RGB}{189,201,225}
\definecolor{colorB}{RGB}{103,169,207}
\definecolor{colorC}{RGB}{ 28,144,153}
\definecolor{colorD}{RGB}{  1,108, 89}

\newcolumntype{R}{>{\columncolor{gray!40}}r}
\newcolumntype{L}{>{\columncolor{gray!40}}l}
\newcolumntype{C}{>{\columncolor{gray!40}}c}
\newcommand{\highlightrow}{\rowcolor{orange!20}}




%table
\usepackage{tabularx,colortbl,xcolor}
\usepackage{multirow}
\usepackage[normalem]{ulem}
\useunder{\uline}{\ul}{}

\newcommand\hy{\textrm{-}}

\usepackage{enumitem}

\usepackage{xparse}% http://ctan.org/pkg/xparse

% \captionsetup[table]{name=Table}
\DeclareGraphicsExtensions{.pdf,.png}


\SetKwInput{KwInput}{Input}
\newcommand{\pluseq}{\mathrel{+}=}
\newcommand{\asteq}{\mathrel{*}=}
\newcommand{\diveq}{\mathrel{/}=}

\usepackage{longtable}
% \usepackage{pgfplots}

\usepackage{url}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{array, caption, makecell, booktabs}
\usepackage{wrapfig}
% \usepackage{floatrow}
\usepackage{comment}
\usepackage{enumitem}
\usepackage{accents}
